A Self-interacting Dark Matter Solution to the Extreme Diversity of Low-mass Halo Properties

The properties of low-mass dark matter (DM) halos appear to be remarkably diverse relative to cold, collisionless DM predictions, even in the presence of baryons. We show that self-interacting DM (SIDM) can simultaneously explain observations of halo diversity at two opposite extremes$-$the inner density profile of the dense substructure perturbing the strong lens galaxy SDSSJ0946+1006 and the rotation curves of isolated, gas-rich ultradiffuse galaxies (UDGs). To achieve this, we present the first cosmological zoom-in simulation featuring strong DM self-interactions in a galaxy group environment centered on a $10^{13}~M_{\mathrm{\odot}}$ host halo. In our SIDM simulation, most surviving subhalos of the group-mass host are deeply core-collapsed, yielding excellent candidates for the observed dense strong-lens perturber. Self-interactions simultaneously create kiloparsec-scale cores in low-concentration isolated halos, which could host the observed UDGs. Our scenario can be further tested with observations of DM structure and galaxies over a wide mass range.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

